Unlocking Spin Dynamics: Spin-Orbit Coupling Driven Spin State Interconversion in Carbazole-Containing TADF Emitters

The determination of transport mechanisms in organic light-emitting diodes (OLEDs) is crucial for optimizing device performance. Magnetic field measurements enable the differentiation of spin state interconversion mechanisms, but data interpretation remains challenging. Here, experimental and theoretical investigations were combined to provide a comprehensive understanding of the underlying processes. This study systematically compares three cyanoarene-based emitters with different singlet-triplet gaps to explore factors influencing reverse intersystem crossing (RISC). The comparison of all-$^1$H and all-$^2$H 4CzIPN isotopologues confirms that RISC is governed by spin-orbit coupling (SOC) rather than hyperfine interactions. Magnetic field-dependent measurements reveal that charge transport in OLED devices is driven by triplet-charge annihilation in 3CzClIPN and 4CzIPN, while triplet-triplet annihilation dominates for 5CzBN. Theoretical calculations further indicate that SOC-mediated RISC in 3CzClIPN and 4CzIPN can additionally occur via a $T_2$ intermediate state with an activation energy distinct from the singlet-triplet energy gap. A temperature-dependent analysis of the devices was conducted to quantify this activation energy and compare it with the computational findings. These findings establish key correlations between activation energy, spin dynamics, and magnetic field effects in TADF emitters, advancing our understanding of excitonic processes in OLEDs.

==> sections/Supplementary_Information.tex <==
\section{Supplementary Information}
\begin{table}
 \caption{Device performance parameters for the devices discussed in this work. The corresponding spectra can be found in Figures \ref{fig:optoelectronic-characterization} and \ref{fig:J-V-Luminance}. The Turn-on voltage was determined for each device at a Luminance (L) of $\mathrm{10 \ cd/m^2}$.}
  \begin{tabular}[htbp]{@{}lllll@{}}
    \hline
    Device & Turn-on voltage / V & Maximum EQE / $\%$ & Maximum L / $\mathrm{cd/m^2}$ & EL peak position / nm\\
    \hline
    3CzClIPN  & ($9.10 \pm 0.46$)  & ($0.11 \pm 0.02$) & ($723.89 \pm 36.68$) & ($549.12 \pm 0.12$)  \\
    4CzIPN  & ($4.22 \pm 0.19$)  & ($0.11 \pm 0.02$) & ($395.08 \pm 19.71$) & ($553.23 \pm 0.12$)  \\
    5CzBN  & ($4.78 \pm 0.24$)  & ($0.13 \pm 0.01$) & ($197.34 \pm 9.85$) & ($511.21 \pm 0.13$)  \\
    3CzClIPN:CBP (1:9)  & ($5.08 \pm 0.25$)  & ($2.76 \pm 0.14$) & ($6689.04 \pm 334.45$) & ($516.32 \pm 0.34$)  \\
    4CzIPN:CBP (1:9) & ($4.44 \pm 0.22$)  & ($2.61 \pm 0.13$) & ($7279.18 \pm 363.96$) & ($549.12 \pm 0.12$)  \\
    5CzBN:CBP (1:9)  & ($5.93 \pm 0.29$)  & ($0.54 \pm 0.03$) & ($1440.93 \pm 72.05$) & ($470.41 \pm 0.14$)  \\
    
    \hline
    \label{tab: Device performance}
  \end{tabular}
\end{table}

\begin{figure}
  \includegraphics[width=\linewidth]{sections/Images/J-V-Luminance-EL-SI.png}
  \caption{Current density and luminance as functions of the applied bias voltage analyzed for (a) the neat films of the materials 3CzClIPN, 4CzIPN, and 5CzBN as well as (b) the corresponding host-guest systems, where the same materials (3CzClIPN, 4CzIPN, and 5CzBN) were employed as guest emitters, embedded in a CBP host matrix. (c) EL spectra for the host-guest systems used at (b). (d) PL spectra for the three emitter molecules 3CzClIPN, 4CzIPN and 5CzBN with the respective full width at half maxima (FWHM).}
  \label{fig:J-V-Luminance}
\end{figure}

\begin{table}   
  \begin{tabular}[htbp]{@{}lll@{}}
  \caption{CIE values for the prsitine molecules 3CzClIPN, 4CzIPN, and 5CzBN, together with their respective host-guest systems}
    \hline
    Device  & CIEx & CIEx \\
    \hline
    3CzClIPN  & 0.401  & 0.564 \\
    4CzIPN  & 0.288  & 0.583 \\
    5CzBN  & 0.272  & 0.470 \\
    3CzClIPN:CBP (1:9)  & 0.258  & 0.554 \\
    4CzIPN:CBP (1:9)  & 0.23  & 0.539 \\
    5CzBN:CBP (1:9)  & 0.166  & 0.032 \\
    
    \hline
    \label{tab: CIE values}
  \end{tabular}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{sections/Images/Magnetoefficiency-B0-HF.png}
    \caption{$\mathrm{B_{0-HF}}$ for 3CzClIPN and 4CzIPN plotted as inset for the Figure \ref{fig:Magnetoefficiency-ramp-data} (b) for a better visibility of the data points}
    \label{fig:Magnetoefficiency-B0-HF}
\end{figure}


\begin{figure}
  \includegraphics[width=\linewidth]{sections/Images/temperature-dependency-full-data.png}
  \caption{Temperature dependent OMC and MEL response for the three TADF-emitter molecules (a) and (d) 3czClIPN, (b) and (e) 4CzIPN, and (c) and (f) 5CzBN.}
  \label{fig:Temp-OMC-MEL-response-full-data}
\end{figure}


\begin{figure}
  \includegraphics[width=\linewidth]{sections/Images/PL-comp.png}
  \caption{Calculated PL spectra for the emitter molecules and the CBP host.}
  \label{fig:computational-PL-sepctra}
\end{figure}

\begin{figure}
  \includegraphics[width=\linewidth]{sections/Images/2D_LIP_full.png}
\caption{Full potential energy surfaces (PES) for LIP between $\mathrm{T_1}$-$\mathrm{T_2}$ conical intersection (CI) and $\mathrm{T_2}$-$\mathrm{S_1}$ minimum energy crossing point (MECP) from different angles. The second dimension corresponds to the displacement of the gradient difference vector (GDV).}
  \label{fig:2D-LIP-full-PES}
\end{figure}

\begin{figure}[h]
\centering
  \includegraphics[width=0.75\textwidth]{sections/Images/1D_LIPS_3Cz.png}
  \caption{Excited state energies at LIPs between selected electronic state minima of 3CzClIPN. (a) shows the $\mathrm{T_1} \rightarrow \mathrm{S_1}$ LIP, (b) $\mathrm{T_2} \rightarrow \mathrm{S_1}$ the LIP, and (c) $\mathrm{T_1} \rightarrow \mathrm{T_2}$ the LIP. Dotted lines correspond to triplet PES, while continuous lines represent singlet state PES.}
  \label{fig:1D-LIPs-3Cz}
\end{figure}

\begin{figure}[h]
\centering
  \includegraphics[width=0.75\textwidth]{sections/Images/1D_LIP_5Cz.png}
  \caption{Excited state energies at LIP between the $\mathrm{T_1}$ and $\mathrm{S_1}$ electronic state minima of 5CzBN. Dotted lines correspond to triplet PES, while continuous lines represent singlet state PES.}
  \label{fig:1D-LIP-5Cz}
\end{figure}


\begin{figure}[h]
\centering
  \includegraphics[width=0.75\textwidth]{sections/Images/Jablonski_3Cz.png}
  \caption{Computational Jablonski diagram for 3CzClIPN.}
  \label{fig:Jablonski-3Cz}
\end{figure}

\begin{figure}[h]
\centering
  \includegraphics[width=0.75\textwidth]{sections/Images/Jablonski_5Cz.png}
  \caption{Computational Jablonski diagram for 5CzBN.}
  \label{fig:Jablonski-5Cz}
\end{figure}

